Parametric Recognizability over the Integers

B\"uchi arithmetic on a fixed integer $k\geq 2$ is the first-order theory of the structure $(\mathbb{Z};0,1,+,V_k,\leq)$, where the binary relation $V_k(x,y)$ is true if and only if $y$ is the greatest power of $k$ dividing $x$. By the B\"uchi-Bruy\`ere theorem, this theory completely describes the sets of integers that are recognizable by finite automata when encoded in the $k$-ary positional number system. Motivated by recent advances in symbolic automata, we study B\"uchi arithmetic with a parametric positional encoding, where $k$ is treated as a variable rather than a fixed constant. We show that this parametric B\"uchi arithmetic provides a logical characterization of a class of parametric symbolic automata over Linear Integer Arithmetic (LIA), thus extending the B\"uchi-Bruy\`ere theorem to the parametric setting. Building on this characterization, we give an algorithm showing that for every first-order sentence $\varphi_t$ in the language of $(\mathbb{Z};0,1,+,V_t,\leq)$, the set of bases $k\geq 2$ where $\varphi_k$ is true is ultimately periodic. The original B\"uchi-Bruy\`ere theorem translates finite automata to the $\exists^*\forall^*$ fragment of B\"uchi arithmetic, while our proof yields the $\exists^*\forall^*\exists^*$ fragment. We trace this discrepancy to the map $x\mapsto k\cdot x$, whose parametric counterpart $x\mapsto t\cdot x$ is not definable in parametric B\"uchi arithmetic: for $\exists^*\forall^*$ sentences $\varphi_t$ in the language of $(\mathbb{Z};0,1,+,x\mapsto t\cdot x,V_t,\leq)$, the existence of a base $k\geq 2$ such that $\varphi_k$ is true is undecidable. Finally, we provide a prototype implementation of both parametric and standard symbolic automata. Experiments indicate that parametric symbolic automata are more efficient when the range of bases $[\alpha..\beta]$ is large, or so is $\alpha$.

==> macros.tex <==
\newcommand{\newextmathcommand}[2]{%
    \newcommand{#1}{\ensuremath{#2}\xspace}
}

\newcommand{\renewextmathcommand}[2]{%
    \renewcommand{#1}{\ensuremath{#2}\xspace}
}

\makeatletter
\newcommand{\labeltext}[2]{%
    #1%
    \@bsphack%
    \csname phantomsection\endcsname
    \def\@currentlabel{#1}{\label{#2}}%
    \@esphack%
}
\makeatother

\makeatletter
\newcommand{\customlabel}[2]{%
    \@bsphack%
    \csname phantomsection\endcsname
    \def\@currentlabel{#1}{\label{#2}}%
    \@esphack%
}
\makeatother

\newcommand{\mathcmt}[1]{\ensuremath{\Lbag\,\text{#1}\,\Rbag}\xspace}

\definecolor{darkblue}{HTML}{0072B2}
\definecolor{vermilion}{HTML}{D55E00}
\definecolor{skyblue}{HTML}{56B4E9}
\definecolor{vscBracketA}{HTML}{0431FA}
\definecolor{vscBracketB}{HTML}{319331}
\definecolor{vscBracketC}{HTML}{7B3814}

\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\green}[1]{\textcolor{skyblue}{#1}}
\newcommand{\brown}[1]{\textcolor{brown}{#1}}
\newcommand{\orange}[1]{\textcolor{vermilion}{#1}}

\newextmathcommand{\N}{\mathbb{N}}
\newextmathcommand{\Np}{\N_+}
\newextmathcommand{\Z}{\mathbb{Z}}
\newextmathcommand{\Q}{\mathbb{Q}}
\newextmathcommand{\R}{\mathbb{R}}

\renewcommand{\vec}{\bm}
\newextmathcommand{\lcm}{{\rm lcm}}
\newcommand{\abs}[1]{\ensuremath{\left|#1\right|}\xspace}
\newcommand{\ceil}[1]{\ensuremath{\left\lceil#1\right\rceil}\xspace}
\newcommand{\floor}[1]{\ensuremath{\left\lfloor#1\right\rfloor}\xspace}
\newextmathcommand{\divs}{\mathrel{|}}
\newextmathcommand{\powerset}{\mathcal{P}}
\newextmathcommand{\Img}{\mathrm{Im}}
\newextmathcommand{\lfp}{\mathrm{lfp}}
\newextmathcommand{\pleq}{\mathbin{\subseteq}}

\newcommand{\norm}[1]{\ensuremath{\lVert #1 \rVert}\xspace}

\newextmathcommand{\ptime}{\textup{\textsc{P}}\xspace}
\newextmathcommand{\fptime}{\textup{\textsc{FP}}\xspace}
\newextmathcommand{\np}{\textup{\textsc{NP}}\xspace}
\newextmathcommand{\fnp}{\textup{\textsc{FNP}}\xspace}
\newextmathcommand{\conp}{\textup{\textsc{coNP}}\xspace}
\newextmathcommand{\pspace}{\textup{\textsc{PSpace}}\xspace}
\newextmathcommand{\nexptime}{\textup{\textsc{NExpTime}}\xspace}
\newextmathcommand{\expspace}{\textup{\textsc{ExpSpace}}\xspace}
\newextmathcommand{\conexp}{\textup{\textsc{coNExp}}\xspace}
\newextmathcommand{\twonexptime}{\textup{\textsc{2NExpTime}}\xspace}
\newextmathcommand{\threeexptime}{\textup{\textsc{3ExpTime}}\xspace}
\newextmathcommand{\tower}{\textup{\textsc{Tower}}\xspace}
\newextmathcommand{\STA}{\textup{\textsc{STA}}\xspace}

\let\temp\phi
\let\phi\varphi
\let\varphi\temp

\newextmathcommand{\Iff}{\Longleftrightarrow}
\newextmathcommand{\Implies}{\Longrightarrow}

\renewextmathcommand{\iff}{\leftrightarrow}

\newextmathcommand{\Formulas}{\mathcal{F}}
\newextmathcommand{\amodel}{\mathfrak{M}}

\newextmathcommand{\theory}{\mathrm{Th}}

\newcommand{\sub}[2]{\ensuremath{[#1\,/\,#2]}\xspace}

\newcommand{\sem}[1]{\ensuremath{\left\llbracket#1\right\rrbracket}\xspace}
\newcommand{\digsem}[1]{\ensuremath{\left\llbracket#1\right\rrbracket^{\#}}\xspace}

\DeclareFontEncoding{LS2}{}{\noaccents@}
\DeclareFontSubstitution{LS2}{stix}{m}{n}
\DeclareSymbolFont{stix@largesymbols}{LS2}{stixex}{m}{n}
\SetSymbolFont{stix@largesymbols}{bold}{LS2}{stixex}{b}{n}
\DeclareMathDelimiter{\lBrace}{\mathopen} {stix@largesymbols}{"E8}%
{stix@largesymbols}{"0E}
\DeclareMathDelimiter{\rBrace}{\mathclose}{stix@largesymbols}{"E9}%
{stix@largesymbols}{"0F}
\newcommand{\multiset}[1]{\ensuremath{\left\lBrace#1\right\rBrace}\xspace}
\newcommand{\defeq}{\coloneqq}
\newcommand{\eqdef}{\defeq}

\newextmathcommand{\Lang}{\mathcal{L}}
\newextmathcommand{\Aut}{\mathcal{A}}

\newextmathcommand{\LangMSD}{\mathcal{L}_{\mathrm{msdf}}}

\newextmathcommand{\PBA}{\textit{PBA}}
\newextmathcommand{\PBAM}{\textit{PBA}[t{\cdot}{}]}
\newextmathcommand{\PBAMA}{\textit{PBA}[t{\cdot}{},\&_t]}
\newextmathcommand{\PPA}{\textit{PrA}[t]}
\newextmathcommand{\kBA}{k\textit{BA}}
\newextmathcommand{\BA}{\textit{BA}}
\newextmathcommand{\pbaformulas}{\Formulas_{\PBA}}
\newextmathcommand{\kbaformulas}{\Formulas_{\kBA}}
\newextmathcommand{\realbases}{\mathscr{B}}
\newextmathcommand{\kBAmodel}{\mathfrak{Ba}}

\newcommand{\tool}{{\tt pbac}\xspace}
\newextmathcommand{\bmin}{\alpha}
\newextmathcommand{\bmax}{\beta}

\newextmathcommand{\PAt}{\textit{PA}t}
\newextmathcommand{\kPAmodel}{\mathfrak{Pa}}

\newextmathcommand{\AutPAt}{\mathcal{A}\mathbf{ut}(\PAt)}

\newextmathcommand{\CEk}{\mathcal{Z}_k}
\newextmathcommand{\Mk}{\mathcal{M}_k}
\newcommand{\intrep}[1]{\ensuremath{\llparenthesis\hspace{1pt}#1\hspace{1pt}\rrparenthesis}\xspace}

\newcommand{\inc}{\texttt{++}}
\newcommand{\dec}{\texttt{{-}{-}}}
\newcommand{\id}{\texttt{id}}

\newcommand{\parmode}{\texttt{par}\xspace}
\newcommand{\symmode}{\texttt{sym}\xspace}

\let\oldmathrm\mathrm
\renewcommand{\mathrm}[1]{\text{\textup{#1}}}

